Extreme Relative Pose Estimation for RGB-D Scans via Scene Completion

Estimating the relative rigid pose between two RGB-D scans of the same underlying environment is a fundamental problem in computer vision, robotics, and computer graphics. Most existing approaches allow only limited maximum relative pose changes since they require considerable overlap between the input scans. We introduce a novel deep neural network that extends the scope to extreme relative poses, with little or even no overlap between the input scans. The key idea is to infer more complete scene information about the underlying environment and match on the completed scans. In particular, instead of only performing scene completion from each individual scan, our approach alternates between relative pose estimation and scene completion. This allows us to perform scene completion by utilizing information from both input scans at late iterations, resulting in better results for both scene completion and relative pose estimation. Experimental results on benchmark datasets show that our approach leads to considerable improvements over state-of-the-art approaches for relative pose estimation. In particular, our approach provides encouraging relative pose estimates even between non-overlapping scans.

==> Tables/table1.bk1.tex <==

\setlength\tabcolsep{1.45pt}
\begin{table*}
\footnotesize
\iffalse

\begin{tabular}{l|ccc|c|ccc|c|ccc|c|ccc|c|ccc|c|ccc|c}
& \multicolumn{8}{c|}{SUNCG} & \multicolumn{8}{c|}{Matterport} & \multicolumn{8}{c}{ScanNet} \\ \hline
&\multicolumn{4}{c|}{Rotation} & \multicolumn{4}{c|}{Trans.} & \multicolumn{4}{c|}{Rotation} & \multicolumn{4}{c|}{Trans.} & \multicolumn{4}{c|}{Rotation} & \multicolumn{4}{c}{Trans.}\\ \hline 
& $\ang{3}$ & $\ang{10}$ & $\ang{45}$ & Mean & $0.1$ & $0.25$& $0.5$ & Mean
& $\ang{3}$ & $\ang{10}$ & $\ang{45}$ & Mean & $0.1$ & $0.25$& $0.5$ & Mean
& $\ang{3}$ & $\ang{10}$ & $\ang{45}$ & Mean & $0.1$ & $0.25$& $0.5$ & Mean
\\ \hline
4PCS([0.5,1]) & 15.5 & 17.8 & 91.1 & 25.05 & 15.9 & 20.5 & 39.1 & 0.66 & 7.5 & 8.5 & 88.7 & 27.49 & 7.5 & 9.4 & 29.1 & 0.77 & 7.8 & 24.4 & 81.9 & 28.76 & 7.8 & 15.0 & 40.0 & 0.74 \\
GReg([0.5,1]) & 84.9 & 91.9 & 93.0 & 10.48 & 85.3 & 86.8 & 89.1 & 0.17 &  83.1 & 89.7 & 92.5 & 11.84 & 84.5 & 88.3 & 90.6 & 0.18 & 59.1 & 85.0 & 89.9 & 15.63 & 82.3 & 86.6 & 90.4 & 0.16\\
CGReg([0.5,1]) & 90.7 & 92.6 & 93.8 & 10.25 & 87.6 & 90.3 & 93.0 & 0.15 & 89.7 & 89.7 & 93.0 & 9.79 & 89.2 & 90.1 & 92.5 & 0.15 & 58.6 & 74.9 & 87.9 & 18.31 & 62.2 & 76.3 & 86.4 & 0.23\\

DL([0.5, 1]) & 0.0 & 0.0 & 15.9 & 81.38 & 0.0 & 1.9 & 8.5 & 1.60 & 0.0 & 0.0 & 9.9 & 83.78 & 0.0 & 3.3 & 6.6 & 1.77 & 0.0 & 0.0 & 29.9 & 61.29 & 0.0 & 0.1 & 0.7 & 3.31\\

Ours-nc.([0.5,1]) & 88.4 & 95.0 & 98.1 & 3.76 & 84.1 & 94.2 & 96.1 & \textbf{0.10} & 88.3 & 97.2 & 97.7 & 3.52 & 90.1 & 96.7 & 98.1 & 0.07 & 57.1 & 82.0 & 90.9 & 13.62 & 62.4 & 78.7 & 87.3 & \textbf{0.22} \\
Ours-nr.([0.5,1]) & 90.3 & 95.7 & 97.3 & 4.12 & 83.7 & 94.6 & 96.9 & \textbf{0.10} & 89.2 & 98.6 & 99.1 & 2.97 & 94.8 & 98.6 & 99.1 & \textbf{0.06} & 47.2 & 72.9 & 90.2 & 14.85 & 55.6 & 73.6 & 82.7 & 0.30 \\
Ours([0.5, 1]) & 89.1 & 96.1 & 98.1 & \textbf{3.58} & 84.5 & 95.0 & 96.5 & \textbf{0.10} & 88.7 & 98.6 & 99.5 & \textbf{2.19} & 86.9 & 94.4 & 98.6 & \textbf{0.06} & 47.0 & 74.3 & 92.6 & \textbf{12.30} & 56.8 & 74.8 & 84.2 & 0.29 \\

\hline
4PCS([0.1,0.5)) & 0.0 & 0.0 & 10.6 & 63.23 & 0.0 & 0.0 & 1.3 & 1.89 & 0.0 & 0.0 & 17.0 & 62.74 & 0.0 & 0.4 & 0.4 & 1.92 & 0.0 & 1.9 & 40.1 & 57.92 & 0.0 & 0.3 & 0.3 & 1.53\\
GReg([0.1,0.5)) & 31.4 & 46.0 & 49.1 & 65.26 & 36.7 & 41.6 & 44.7 & 1.30 & 18.9 & 29.0 & 36.7 & 70.48 & 25.9 & 29.0 & 31.7 & 1.61 & 10.9 & 25.0 & 32.1 & 90.26 & 18.3 & 22.4 & 24.0 & 1.30\\
CGReg([0.1,0.5]) & 43.8 & 47.3 & 50.0 & 65.41 & 38.9 & 41.2 & 45.1 & 2.25 & 31.3 & 32.0 & 37.1 & 74.14 & 30.9 & 30.9 & 32.0 & 1.69 & 10.6 & 18.3 & 32.7 & 89.94 & 11.5 & 15.7 & 21.5 & 1.41\\

DL([0.1, 0.5)) & 0.0 & 0.0 & 8.0 & 93.93 & 0.0 & 1.8 & 4.0 & 2.06 & 0.0 & 0.0 & 8.5 & 94.34 & 0.0 & 0.4 & 2.7 & 2.25 & 0.0 & 0.0 & 7.5 & 92.09 & 0.0 & 0.0 & 0.0 & 4.03\\

Ours-nc.([0.1,0.5]) & 46.0 & 62.8 & 69.5 & 35.37 & 36.7 & 56.6 & 64.2 & 0.90 & 52.9 & 73.4 & 81.9 & 23.88 & 48.3 & 62.2 & 70.3 & 0.60 & 13.2 & 32.9 & 52.0 & 56.94 & 17.8 & 29.2 & 37.5 & 0.98\\
Ours-nr.([0.1,0.5]) & 61.5 & 80.5 & 82.3 & 22.16 & 42.9 & 71.2 & 80.5 & 0.59 & 48.3 & 74.5 & 83.8 & 24.42 & 49.4 & 65.6 & 76.8 & 0.53 & 8.6 & 30.2 & 56.0 & 51.17 & 11.1 & 26.2 & 38.8 & 1.08\\
Ours([0.1,0.5)) & 68.6 & 82.3 & 85.0 & \textbf{20.28} & 45.1 & 76.5 & 82.7 & \textbf{0.54}
  & 52.1 & 81.5 & 89.2 & \textbf{16.74} & 49.4 & 69.5 & 77.6 & \textbf{0.46} & 11.1 & 33.5 & 64.3 & \textbf{44.37} & 12.6 & 28.3 & 40.3 & \textbf{0.98}\\ \hline

DL([0.0, 0.1)) & 0.0 & 0.0 & 1.7 & 117.48 & 0.0 & 4.1 & 14.0 & 1.49 & 0.0 & 0.0 & 2.1 & 125.86 & 0.0 & 0.2 & 2.1 & 2.83 & 0.0 & 0.0 & 0.0 & 130.43 & 0.0 & 0.0 & 0.0 & 5.37\\

Ours-nc.([0.0,0.1]) & 3.4 & 6.9 & 14.7 & 110.09 & 0.0 & 0.9 & 14.7 & 1.51 & 0.9 & 5.1 & 12.3 & 118.25 & 0.0 & 0.0 & 0.0 & 3.16 & 1.2 & 5.8 & 16.3 & 105.74 & 0.0 & 0.0 & 1.9 & 1.93\\
Ours-nr.([0.0,0.1]) & 6.0 & 18.1 & 30.2 & 86.93 & 2.6 & 11.2 & 26.7 & 1.20 & 1.1 & 6.2 & 21.2 & 104.26 & 0.2 & 0.9 & 3.8 & 2.61 & 0.8 & 7.4 & 30.6 & 80.88 & 0.4 & 3.9 & 8.1 & \textbf{1.69}\\
Ours([0.0,0.1)) & 7.8 & 24.1 & 37.9 & \textbf{80.66} & 1.7 & 14.7 & 30.2 & \textbf{1.04} & 0.9 & 11.2 & 25.4 & \textbf{96.12} & 0.2 & 2.1 & 6.8 & \textbf{2.44}
 & 0.8 & 10.5 & 34.9 & \textbf{76.79} & 0.0 & 3.5 & 12.8 & 1.75\\ 
 Identity([0.0,0.1)) &  &  &  & 116.21 &  &  &  & 1.76 &  &  &  & 131.09 &  &  & 
 & 03.41 &  &  &  & 82.48 &  &  & & 2.09\\ 
 \hline

\end{tabular}
\caption{\small{Benchmark evaluation on our approach and baseline approaches. Ours-nc and Ours-nr stand for ours method with completion module and recurrent module removed, respectively. For the rotation component, we show the percentage of pairs whose angular deviations fall within $3^{\circ}$,$10^{\circ}$, and $45^{\circ}$, respectively. For the translation component, we show the percentage of pairs whose translation deviations fall within $0.1m$,$0.25m$,$0.5m$
%$0.1d$, $0.15d$, and $0.5d$, where $d$ is the diameter of each scan. 
We also show the mean errors. In addition, we show statistics for pairs of scans whose overlapping ratios fall into three
intervals, namely, [50\%, 100\%], [10\%, 50\%], and [0\%, 10\%]. }}
\label{Table:Benchmark:Evaluation}
\vspace{-0.05in}
\end{table*}

\fi 


\begin{tabular}{l|ccc|c|ccc|c|ccc|c|ccc|c|ccc|c|ccc|c}
& \multicolumn{8}{c|}{SUNCG} & \multicolumn{8}{c|}{Matterport} & \multicolumn{8}{c}{ScanNet} \\ \hline
&\multicolumn{4}{c|}{Rotation} & \multicolumn{4}{c|}{Trans.} & \multicolumn{4}{c|}{Rotation} & \multicolumn{4}{c|}{Trans.} & \multicolumn{4}{c|}{Rotation} & \multicolumn{4}{c}{Trans.}\\ \hline 
& $\ang{3}$ & $\ang{10}$ & $\ang{45}$ & Mean & $0.1$ & $0.25$& $0.5$ & Mean
& $\ang{3}$ & $\ang{10}$ & $\ang{45}$ & Mean & $0.1$ & $0.25$& $0.5$ & Mean
& $\ang{3}$ & $\ang{10}$ & $\ang{45}$ & Mean & $0.1$ & $0.25$& $0.5$ & Mean
\\ \hline
4PCS([0.5,1]) & 64.3 & 83.7 & 87.6 & 21.0 & 68.2 & 74.4 & 79.0 & 0.30 & 42.7 & 65.7 & 80.3 & 33.4 & 52.6 & 64.3 & 69.0 & 0.46 & 25.3 & 48.7 & 80.1 & 31.2 & 36.9 & 43.2 & 59.8 & 0.52 \\
GReg([0.5,1]) & 85.9 & 91.9 & 94.1 & 10.3 & 86.9 & 89.3 & 90.7 & 0.16 &  80.8 & 89.2 & 92.1 & 12.0 & 84.8 & 88.5 & 90.6 & 0.17 & 58.9 & 84.4 & 88.8 & 16.3 & 81.7 & 85.8 & 88.6 & \textbf{0.19}\\
CGReg([0.5,1]) & 90.8 & 92.9 & 93.9 & 9.8 & 87.3 & 90.7 & 92.8 & 0.13 & 90.3 & 90.8 & 93.1 & 10.1 & 89.4 & 89.6 & 91.6 & 0.14 & 59.0 & 75.7 & 88.1 & 18.0 & 62.1 & 77.7 & 86.9 & 0.23\\

DL([0.5, 1]) & 0.0 & 0.0 & 15.9 & 81.4 & 0.0 & 1.9 & 8.5 & 1.60 & 0.0 & 0.0 & 9.9 & 83.8 & 0.0 & 3.3 & 6.6 & 1.77 & 0.0 & 0.0 & 30.0 & 61.3 & 0.0 & 0.1 & 0.7 & 3.31\\

Ours-nc.([0.5,1]) & 88.1 & 94.5 & 97.5 & 4.4 & 82.4 & 92.5 & 95.9 & 0.11 & 90.9 & 98.0 & 99.2 & 1.9 & 93.8 & 97.3 & 99.1 & \textbf{0.04} & 56.6 & 80.9 & 90.1 & 14.3 & 66.5 & 79.7 & 86.1 & 0.23 \\
Ours-nr.([0.5,1]) & 90.9 & 96.0 & 97.8 & 4.1 & 84.5 & 94.9 & 96.8 & \textbf{0.10} & 87.7 & 97.4 & 98.8 & 3.0 & 90.0 & 94.8 & 97.5 & 0.07 & 52.4 & 78.9 & 91.1 & 13.4 & 64.4 & 78.0 & 86.5 & 0.23 \\
Ours([0.5, 1]) & 90.1 & 96.2 & 97.8 & \textbf{3.9} & 83.7 & 94.5 & 96.6 & \textbf{0.10} & 89.6 & 98.7 & 99.6 & \textbf{1.8} & 92.5 & 96.7 & 98.5 & 0.05 & 53.3 & 79.9 & 91.3 & \textbf{13.0} & 66.4 & 79.6 & 86.1 & 0.23 \\

\hline
4PCS([0.1,0.5)) & 4.9 & 10.6 & 13.7 & 113.0 & 4.0 & 5.3 & 7.1 & 1.99 & 4.2 & 16.2 & 25.9 & 87.0 & 5.0 & 8.1 & 10.0 & 2.19 & 1.5 & 7.1 & 30.0 & 82.2 & 2.5 & 3.1 & 3.1 & 1.63\\
GReg([0.1,0.5)) & 35.1 & 45.4 & 50.3 & 64.1 & 35.8 & 40.3 & 43.6 & 1.29 & 19.2 & 26.8 & 34.9 & 73.8 & 24.2 & 27.2 & 28.4 & 1.68 & 11.4 & 25.0 & 33.3 & 86.5 & 18.1 & 21.7 & 23.4 & 1.31\\
CGReg([0.1,0.5]) & 46.4 & 48.5 & 51.0 & 63.4 & 40.2 & 42.7 & 46.0 & 1.34 & 28.5 & 29.3 & 35.9 & 73.9 & 28.1 & 28.3 & 29.5 & 1.99 & 11.8 & 20.0 & 32.9 & 88.2 & 11.6 & 16.0 & 21.0 & 1.36\\

DL([0.1, 0.5)) & 0.0 & 0.0 & 8.0 & 94.0 & 0.0 & 1.8 & 4.0 & 2.06 & 0.0 & 0.0 & 8.5 & 94.3 & 0.0 & 0.4 & 2.7 & 2.25 & 0.0 & 0.0 & 7.5 & 92.1 & 0.0 & 0.0 & 0.0 & 4.03\\

Ours-nc.([0.1,0.5]) & 47.4 & 63.5 & 71.0 & 32.7 & 35.4 & 55.9 & 64.3 & 0.87 & 57.0 & 75.9 & 83.5 & 22.5 & 52.5 & 66.4 & 74.6 & 0.53 & 13.8 & 37.1 & 56.6 & 54.9 & 18.2 & 31.3 & 41.5 & 0.97\\
Ours-nr.([0.1,0.5]) & 62.3 & 79.6 & 82.9 & 21.6 & 43.1 & 70.4 & 80.0 & 0.58 & 50.9 & 73.1 & 83.5 & 22.4 & 47.0 & 65.2 & 74.6 & 0.55 & 12.2 & 35.4 & 62.0 & 49.9 & 18.9 & 33.1 & 45.7 & 0.93\\
Ours([0.1,0.5)) & 66.2 & 83.0 & 85.1 & \textbf{20.1} & 43.8 & 73.0 & 83.0 & \textbf{0.52}
  & 54.1 & 81.5 & 88.6 & \textbf{16.3} & 51.4 & 70.0 & 81.0 & \textbf{0.45} & 13.3 & 38.8 & 64.3 & \textbf{47.4} & 20.0 & 33.6 & 47.5 & \textbf{0.90}\\ \hline

DL([0.0, 0.1)) & 0.0 & 0.0 & 2.1 & 115.4 & 0.0 & 1.4 & 4.3 & 2.23 & 0.0 & 0.0 & 2.1 & 125.9 & 0.0 & 0.2 & 2.1 & 2.83 & 0.0 & 0.0 & 0.0 & 130.4 & 0.0 & 0.0 & 0.0 & 5.37\\

Ours-nc.([0.0,0.1]) & 2.8 & 7.0 & 14.1 & 101.2 & 0.1 & 0.6 & 5.1 & 2.22 & 1.5 & 5.1 & 12.6 & 116.4 & 0.1 & 0.1 & 0.9 & 3.10 & 0.2 & 4.7 & 17.0 & 98.7 & 0.1 & 0.4 & 2.2 & 1.93\\
Ours-nr.([0.0,0.1]) & 13.1 & 27.0 & 32.7 & 83.9 & 2.9 & 15.8 & 28.5 & 1.79 & 1.4 & 10.8 & 26.9 & 93.9 & 0.2 & 2.0 & 6.9 & 2.35 & 0.8 & 8.7 & 29.7 & 84.5 & 0.4 & 1.8 & 7.5 & 1.71\\
Ours([0.0,0.1)) & 15.1 & 32.0 & 37.3 & \textbf{79.9} & 4.5 & 21.1 & 33.8 & \textbf{1.67} & 2.8 & 17.0 & 30.3 & \textbf{87.9} & 0.2 & 3.5 & 11.8 & \textbf{2.20}
 & 0.7 & 8.0 & 31.0 & \textbf{81.8} & 0.2 & 2.2 & 9.0 & \textbf{1.64}\\ 
 Identity([0.0,0.1)) &  &  &  & 103.8 &  &  &  & 2.37 &  &  &  & 131.1 &  &  & 
 & 3.20 &  &  &  & 82.5 &  &  & & 1.96\\ 
 \hline

\end{tabular}
\caption{\small{Benchmark evaluation on our approach and baseline approaches. Ours-nc and Ours-nr stand for ours method with completion module and recurrent module removed, respectively. For the rotation component, we show the percentage of pairs whose angular deviations fall within $3^{\circ}$,$10^{\circ}$, and $45^{\circ}$, respectively. For the translation component, we show the percentage of pairs whose translation deviations fall within $0.1m$,$0.25m$,$0.5m$
%$0.1d$, $0.15d$, and $0.5d$, where $d$ is the diameter of each scan. 
We also show the mean errors. In addition, we show statistics for pairs of scans whose overlapping ratios fall into three
intervals, namely, [50\%, 100\%], [10\%, 50\%], and [0\%, 10\%]. Average numbers are reported for 10 repeated runs on test sets.}}
\label{Table:Benchmark:Evaluation}
\vspace{-0.05in}
\end{table*}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\Ls}{\mathcal{L}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\let\ab\allowbreak

